Modeling Human-AI Team Decision Making

AI and humans bring complementary skills to group deliberations. Modeling this group decision making is especially challenging when the deliberations include an element of risk and an exploration-exploitation process of appraising the capabilities of the human and AI agents. To investigate this question, we presented a sequence of intellective issues to a set of human groups aided by imperfect AI agents. A group's goal was to appraise the relative expertise of the group's members and its available AI agents, evaluate the risks associated with different actions, and maximize the overall reward by reaching consensus. We propose and empirically validate models of human-AI team decision making under such uncertain circumstances, and show the value of socio-cognitive constructs of prospect theory, influence dynamics, and Bayesian learning in predicting the behavior of human-AI groups.

==> Human-agent teaming/proof.tex <==
\section*{Proofs}
\begin{lemma}\label{lem:avg2nd}
For any $0 \leq x_1 \leq x_2 \leq 1$ and $0 \leq y_2 \leq y_1 \leq 1$, \[-(y_1 \ln x_1 + y_2 \ln x_2) \geq -(y_1 + y_2) \ln \frac{x_1+x_2}{2} \]
\end{lemma}

\begin{proof}
Since the function $\ln(x)$ is concave,

\begin{align*}
\ln \frac{x_1+x_2}{2} &\geq \frac{1}{2}\ln x_1 + \frac{1}{2}\ln x_2\\
(y_1 + y_2) \ln \frac{x_1+x_2}{2} &\geq \frac{y_1+y_2}{2}\ln x_1 + \frac{y_1+y_2}{2}\ln x_2\\
&= y_1 \ln x_1 + y_2 \ln x_2 + \frac{y_2 - y_1}{2}\ln x_1 + \frac{y_1 - y_2}{2}\ln x_2\\
&= y_1 \ln x_1 + y_2 \ln x_2 + \frac{y_2 - y_1}{2}(\ln x_1 - \ln x_2)\\
&= y_1 \ln x_1 + y_2 \ln x_2 + \frac{y_2 - y_1}{2}\ln \frac{x_1}{x_2}\\
&\geq y_1 \ln x_1 + y_2 \ln x_2
\end{align*}
\end{proof}

\begin{lemma}
Given a distribution $p$ with a total mass $m_p=\Sigma_i p(i)$, among all distributions with a mass of $m_q$, the distribution that minimizes $-\Sigma_i p(i)\ln q(i)$ and  $-\Sigma_i q(i)\ln p(i)$, is $q^* = \frac{m_q}{m_p}p$.
\end{lemma}

\begin{proof}

Consider any $q$ with $m_q=\Sigma_i q(i)$. 
\begin{align*}
    - \Sigma_i p_i \ln q_i &=     - \Sigma_i p_i \ln \frac{q_i}{m_q} - \Sigma_i p_i \ln m_q\\
    &= - m_p\Sigma_i \frac{p_i}{m_p} \ln \frac{q_i}{m_q} - m_p \ln m_q\\
    &= m_p H(\frac{p}{m_p}, \frac{q}{m_q}) - m_p \ln m_q\\ 
    &\geq m_p H(\frac{p}{m_p}) - m_p \ln m_q\\ 
\end{align*}

Since $q^* = \frac{m_q}{m_p}p$, it follows that
\begin{align*}
    - \Sigma_i p_i \ln q^*_i &= m_p H(\frac{p}{m_p}, \frac{q}{m_q}) - m_p \ln m_q\\ 
    &= m_p H(\frac{p}{m_p}, \frac{m_q}{m_p} \frac{p}{m_q}) - m_p \ln m_q\\
    &= m_p H(\frac{p}{m_p}, \frac{p}{m_p}) - m_p \ln m_q\\    
    &= m_p H(\frac{p}{m_p}) - m_p \ln m_q\\ 
\end{align*}
Therefore, 
$    - \Sigma_i p(i) \ln q_i \geq    - \Sigma_i p(i) \ln q^*_i$. 
Similarly,
\begin{align*}
    - \Sigma_i q_i \ln p_i &=     - \Sigma_i q_i \ln \frac{p_i}{m_p} - \Sigma_i q_i \ln m_p\\
    &= - m_q\Sigma_i \frac{q_i}{m_q} \ln \frac{p_i}{m_p} - m_q \ln m_p\\
    &= m_q H(\frac{q}{m_q}, \frac{p}{m_p}) - m_q \ln m_p\\ 
    &\geq m_q H(\frac{q}{m_q}) - m_q \ln m_p\\ 
\end{align*}

Since $q^* = \frac{m_q}{m_p}p$, it follows that
\begin{align*}
    - \Sigma_i q_i \ln p^*_i &= m_q H(\frac{q}{m_q}, \frac{p}{m_p}) - m_q \ln m_p\\ 
    &= m_q H(\frac{q}{m_q}, \frac{m_p}{m_q} \frac{q}{m_p}) - m_q \ln m_p\\
    &= m_q H(\frac{q}{m_q}, \frac{q}{m_q}) - m_q \ln m_p\\    
    &= m_q H(\frac{q}{m_q}) - m_q \ln m_p\\ 
\end{align*}
Therefore, 
$    - \Sigma_i q(i) \ln p_i \geq    - \Sigma_i q^*(i) \ln p_i$. 
\end{proof}

The above two lemmas imply that given a probability distribution $p$ with a maximum value at $i$, in order to construct a distribution $q$ whose maximum value is constrained to be at $j \neq i$ and whose cross-entropy $H(p,q)$ is minimized with respect to $p$, values in $q$ must be chosen so that the values in positions $i$ and $j$ are equal and the rest of the mass in $q$ is distributed according to the shape of $p$. The following theorem establishes the optimal $q$ based on these considerations.

\begin{theorem}
Given a distribution $p$, $p_i \geq p_k, \forall k$,  Let $m_p^*$ be the total mass of $p$ outside the entries $i$ and $j$, and $p_f = \max_{ k \notin \lbrace i,j\rbrace }p_k$.
Construct a distribution $q$ as follows:
$q_i = q_j = \eta$, $\forall k, k \neq i, k \neq j, q_k = (1-2\eta)\frac{p_k}{m_p^*}$. When $\eta = \max\big(\frac{1}{2+(m_p^*/q_f)},\frac{p_i+p_j}{2}\big), q_k = p_k\frac{(1-2\eta)}{m_p^*} \forall k \notin \lbrace i,j\rbrace$ , the cross-entropy between $p$ and $q$, $H(p,q)$, is minimized. 
\label{the:h_q_p}
\end{theorem}

% \begin{proof}
% \[H(p,q) = - (p_i + p_j) \ln \alpha + m_p^* H(\frac{p^*}{m_p^*}) -m_p^*\ln (1-2\alpha)\]\\
% \begin{align*}
% \frac{d H(p,q)}{d \alpha} &= - \frac{p_i + p_j}{\alpha} + 2 \frac{m_p^*}{1-2\alpha}
% \end{align*}
% This means that at the optimal value,
% \[\alpha = \frac{p_i+p_j}{2(m_p^*+p_i+p_j)}\].

% Missing: show that this is a minima.
% \end{proof}

\begin{proof}
\begin{align*}
H(p,q) &= - (p_i + p_j) \ln \eta -\sum_{k, \forall k, k \neq i, k \neq j}p_k\ln(q_k)\\
&=- (p_i + p_j) \ln \eta-\sum_{k, \forall k, k \neq i, k \neq j}p_k\ln\left(\frac{(1-2\eta)p_k}{m_p^*}\right)\\
\frac{d H(p,q)}{d \eta} &= - \frac{p_i + p_j}{\eta} + \frac{2\sum_{k, \forall k, k \neq i, k \neq j}p_k}{1-2\eta}\\
&=- \frac{p_i + p_j}{\eta}+\frac{2m_p^*}{1-2\eta}
\end{align*}

This means that at the optimal value,
\[\eta = \frac{p_i+p_j}{2}\]. 


Since the second derivative at all feasible $\eta$, 
\[\frac{d^2 H(p,q)}{d \eta^2} = \frac{p_i + p_j}{\eta^2} + \frac{4m_p^*}{(1-2\eta)^2} > 0\]

the cross-entropy is convex and the minimum is achieved at $\eta$. If $\eta \geq q_k,\forall k \neq i, k \neq j $, the solution obeys the constraints and the minimum cross-entropy is achieved at the optimal $\eta$. Otherwise, the minimum cross entropy is either achieved at the minimum or maximum possible value of $\eta$. Since $\eta > (p_i+p_j)/2$, the minimum value of $H(p,q)$ occurs at the minimum valid value of $\eta$.  This occurs when $\eta = \max\limits_{k,k\neq i, k\neq j}p_k = p_f$ for some index $f$. 
Put $r=\frac{\max\limits_{k,k\neq i, k\neq j} p_k}{m_p^*}$ so at its minimum valid value,
\[\eta = q_f = p_f \frac{m_q^*}{m_p^*} = \frac{1}{2+(1/r)}\]

%Otherwise, we optimize $H(p,q)$ as a function of $\eta$ over the range of possible values

%and $\beta$ is a weight parameter. We move a quantity $(1-2\eta)\beta$ of mass that is outside entries $q_i$ and $q_j$ to $q_i$ and $q_j$, such that entries $q_i$, $q_j$ and $q_m$ have the same quantity of mass, where $m$ is the index of $\max q_k, \forall k, k \neq i, k \neq j$. 

%\begin{align*}
%\frac{(1-2\eta)\beta}{2}+\eta &= (1-2\eta)(1-\beta)r\\
%\beta&=\frac{2r}{2r+1}-\frac{2\eta}{(2r+1)(1-2\eta)}
%\end{align*}
%Then, η
%we have $q_i = q_j \geq \frac{r}{2r+1}$, $q_k \leq (1-\frac{2r}{2r+1})\frac{p_k}{\Sigma_{l \neq i, j} p_l}, \forall k, k \neq i, k \neq j$. 
Hence, constructing $q$ with $\eta = \max\big(\frac{1}{2+(m_p^*/p_f)},\frac{p_i+p_j}{2}\big), q_k = p_k\frac{(1-2\eta)}{m_p^*}, \forall k \notin \lbrace i,j\rbrace$ is an optimal solution.
\end{proof}

% \newpage

\begin{lemma}
For any $0 \leq x_1 \leq x_2 \leq 1$ and $0 \leq y_2 \leq y_1 \leq 1$, \[-(x_1 \ln y_1 + x_2 \ln y_2) \geq -(\frac{x_1+x_2}{2} \ln y_1 + \frac{x_1+x_2}{2} \ln y_2) \]
\label{lemma1:v2}
\end{lemma}

\begin{proof}
\begin{align*}
-(x_1 \ln y_1 + x_2 \ln y_2) + (\frac{x_1+x_2}{2} \ln y_1 + \frac{x_1+x_2}{2} \ln y_2) &= \frac{x_2-x_1}{2} \ln y_1 - \frac{x_2-x_1}{2} \ln y_2\\
&= \frac{x_2-x_1}{2} (\ln y_1 - \ln y_2)\\
&\geq 0
\end{align*}
\end{proof}
%current
The above lemma implies that given a probability distribution $p$ with a maximum value at $j$, in order to construct a distribution $q$ whose maximum value is constrained to be at $i \neq j$ and whose cross-entropy $H(q,p)$ is minimized with respect to $q$, values in $q$ must be chosen so that the values in positions $i$ and $j$ are equal. The following theorem establishes the optimal $p$ based on these considerations.

\begin{theorem}
Given a distribution $p$, $p_j \geq p_k, \forall k$. We are asked to construct a distribution $q$ that minimizes the cross entropy $H(q,p)$ under the constraint that $q_i \geq q_k, \forall k$. Consider the  entries $l, l \neq i, l \neq j$ in $p$ that are larger than $\sqrt{p_i p_j}$. The optimal $q$ then is obtained by setting $i$, $j$, and all such entries $l$ to an equal value and all other entries in $q$ to 0.
\label{the:h_p_q}
\end{theorem}
\begin{proof}
Lemma~\ref{lemma1:v2} implies that $q_i = q_j \geq p_k, k \neq i, k \neq j$. Next, we consider which of the remaining entries in $q$ should be non-zero. Clearly, any such entry cannot exceed $q_i$. Consider when a transfer of mass $\alpha$ from $q_i$ and $q_j$ to $q_k$ reduces the entropy $H(q,p)$. For this, we must have\\
\begin{align*}
    - \alpha \ln p_k &< - (\frac{\alpha}{2} \ln p_i + \frac{\alpha}{2} \ln p_j)\\
     -  \ln p_k &< - \frac{1}{2} \ln (p_i p_j)\\
     -  \ln p_k &< - \ln \sqrt{p_i p_j}\\  
     p_k &> \sqrt{p_i p_j}\\
\end{align*}

The maximum mass that can be moved to $p_k$ cannot exceed the value $q_i$. This means that at the optimal $q$,  $q_i$, $q_j$, and all such entries $l$ for which $p_l > \sqrt{p_i p_j}$ are equal to each other, and the rest of the entries in $q$ are 0.

\end{proof}

==> proof.tex <==
\section*{Proofs}
\begin{lemma}\label{lem:avg2nd}
For any $0 \leq x_1 \leq x_2 \leq 1$ and $0 \leq y_2 \leq y_1 \leq 1$, \[-(y_1 \ln x_1 + y_2 \ln x_2) \geq -(y_1 + y_2) \ln \frac{x_1+x_2}{2} \]
\end{lemma}

\begin{proof}
Since the function $\ln(x)$ is concave,

\begin{align*}
\ln \frac{x_1+x_2}{2} &\geq \frac{1}{2}\ln x_1 + \frac{1}{2}\ln x_2\\
(y_1 + y_2) \ln \frac{x_1+x_2}{2} &\geq \frac{y_1+y_2}{2}\ln x_1 + \frac{y_1+y_2}{2}\ln x_2\\
&= y_1 \ln x_1 + y_2 \ln x_2 + \frac{y_2 - y_1}{2}\ln x_1 + \frac{y_1 - y_2}{2}\ln x_2\\
&= y_1 \ln x_1 + y_2 \ln x_2 + \frac{y_2 - y_1}{2}(\ln x_1 - \ln x_2)\\
&= y_1 \ln x_1 + y_2 \ln x_2 + \frac{y_2 - y_1}{2}\ln \frac{x_1}{x_2}\\
&\geq y_1 \ln x_1 + y_2 \ln x_2
\end{align*}
\end{proof}

\begin{lemma}
Given a distribution $p$ with a total mass $m_p=\Sigma_i p(i)$, among all distributions with a mass of $m_q$, the distribution that minimizes $-\Sigma_i p(i)\ln q(i)$ and  $-\Sigma_i q(i)\ln p(i)$, is $q^* = \frac{m_q}{m_p}p$.
\end{lemma}

\begin{proof}

Consider any $q$ with $m_q=\Sigma_i q(i)$. 
\begin{align*}
    - \Sigma_i p_i \ln q_i &=     - \Sigma_i p_i \ln \frac{q_i}{m_q} - \Sigma_i p_i \ln m_q\\
    &= - m_p\Sigma_i \frac{p_i}{m_p} \ln \frac{q_i}{m_q} - m_p \ln m_q\\
    &= m_p H(\frac{p}{m_p}, \frac{q}{m_q}) - m_p \ln m_q\\ 
    &\geq m_p H(\frac{p}{m_p}) - m_p \ln m_q\\ 
\end{align*}

Since $q^* = \frac{m_q}{m_p}p$, it follows that
\begin{align*}
    - \Sigma_i p_i \ln q^*_i &= m_p H(\frac{p}{m_p}, \frac{q}{m_q}) - m_p \ln m_q\\ 
    &= m_p H(\frac{p}{m_p}, \frac{m_q}{m_p} \frac{p}{m_q}) - m_p \ln m_q\\
    &= m_p H(\frac{p}{m_p}, \frac{p}{m_p}) - m_p \ln m_q\\    
    &= m_p H(\frac{p}{m_p}) - m_p \ln m_q\\ 
\end{align*}
Therefore, 
$    - \Sigma_i p(i) \ln q_i \geq    - \Sigma_i p(i) \ln q^*_i$. 
Similarly,
\begin{align*}
    - \Sigma_i q_i \ln p_i &=     - \Sigma_i q_i \ln \frac{p_i}{m_p} - \Sigma_i q_i \ln m_p\\
    &= - m_q\Sigma_i \frac{q_i}{m_q} \ln \frac{p_i}{m_p} - m_q \ln m_p\\
    &= m_q H(\frac{q}{m_q}, \frac{p}{m_p}) - m_q \ln m_p\\ 
    &\geq m_q H(\frac{q}{m_q}) - m_q \ln m_p\\ 
\end{align*}

Since $q^* = \frac{m_q}{m_p}p$, it follows that
\begin{align*}
    - \Sigma_i q_i \ln p^*_i &= m_q H(\frac{q}{m_q}, \frac{p}{m_p}) - m_q \ln m_p\\ 
    &= m_q H(\frac{q}{m_q}, \frac{m_p}{m_q} \frac{q}{m_p}) - m_q \ln m_p\\
    &= m_q H(\frac{q}{m_q}, \frac{q}{m_q}) - m_q \ln m_p\\    
    &= m_q H(\frac{q}{m_q}) - m_q \ln m_p\\ 
\end{align*}
Therefore, 
$    - \Sigma_i q(i) \ln p_i \geq    - \Sigma_i q^*(i) \ln p_i$. 
\end{proof}

The above two lemmas imply that given a probability distribution $p$ with a maximum value at $i$, in order to construct a distribution $q$ whose maximum value is constrained to be at $j \neq i$ and whose cross-entropy $H(p,q)$ is minimized with respect to $p$, values in $q$ must be chosen so that the values in positions $i$ and $j$ are equal and the rest of the mass in $q$ is distributed according to the shape of $p$. The following theorem establishes the optimal $q$ based on these considerations.

\begin{theorem}
Given a distribution $p$, $p_i \geq p_k, \forall k$,  Let $m_p^*$ be the total mass of $p$ outside the entries $i$ and $j$, and $p_f = \max_{ k \notin \lbrace i,j\rbrace }p_k$.
Construct a distribution $q$ as follows:
$q_i = q_j = \eta$, $\forall k, k \neq i, k \neq j, q_k = (1-2\eta)\frac{p_k}{m_p^*}$. When $\eta = \max\big(\frac{1}{2+(m_p^*/q_f)},\frac{p_i+p_j}{2}\big), q_k = p_k\frac{(1-2\eta)}{m_p^*} \forall k \notin \lbrace i,j\rbrace$ , the cross-entropy between $p$ and $q$, $H(p,q)$, is minimized. 
\label{the:h_q_p}
\end{theorem}

% \begin{proof}
% \[H(p,q) = - (p_i + p_j) \ln \alpha + m_p^* H(\frac{p^*}{m_p^*}) -m_p^*\ln (1-2\alpha)\]\\
% \begin{align*}
% \frac{d H(p,q)}{d \alpha} &= - \frac{p_i + p_j}{\alpha} + 2 \frac{m_p^*}{1-2\alpha}
% \end{align*}
% This means that at the optimal value,
% \[\alpha = \frac{p_i+p_j}{2(m_p^*+p_i+p_j)}\].

% Missing: show that this is a minima.
% \end{proof}

\begin{proof}
\begin{align*}
H(p,q) &= - (p_i + p_j) \ln \eta -\sum_{k, \forall k, k \neq i, k \neq j}p_k\ln(q_k)\\
&=- (p_i + p_j) \ln \eta-\sum_{k, \forall k, k \neq i, k \neq j}p_k\ln\left(\frac{(1-2\eta)p_k}{m_p^*}\right)\\
\frac{d H(p,q)}{d \eta} &= - \frac{p_i + p_j}{\eta} + \frac{2\sum_{k, \forall k, k \neq i, k \neq j}p_k}{1-2\eta}\\
&=- \frac{p_i + p_j}{\eta}+\frac{2m_p^*}{1-2\eta}
\end{align*}

This means that at the optimal value,
\[\eta = \frac{p_i+p_j}{2}\]. 


Since the second derivative at all feasible $\eta$, 
\[\frac{d^2 H(p,q)}{d \eta^2} = \frac{p_i + p_j}{\eta^2} + \frac{4m_p^*}{(1-2\eta)^2} > 0\]

the cross-entropy is convex and the minimum is achieved at $\eta$. If $\eta \geq q_k,\forall k \neq i, k \neq j $, the solution obeys the constraints and the minimum cross-entropy is achieved at the optimal $\eta$. Otherwise, the minimum cross entropy is either achieved at the minimum or maximum possible value of $\eta$. Since $\eta > (p_i+p_j)/2$, the minimum value of $H(p,q)$ occurs at the minimum valid value of $\eta$.  This occurs when $\eta = \max\limits_{k,k\neq i, k\neq j}p_k = p_f$ for some index $f$. 
Put $r=\frac{\max\limits_{k,k\neq i, k\neq j} p_k}{m_p^*}$ so at its minimum valid value,
\[\eta = q_f = p_f \frac{m_q^*}{m_p^*} = \frac{1}{2+(1/r)}\]

%Otherwise, we optimize $H(p,q)$ as a function of $\eta$ over the range of possible values

%and $\beta$ is a weight parameter. We move a quantity $(1-2\eta)\beta$ of mass that is outside entries $q_i$ and $q_j$ to $q_i$ and $q_j$, such that entries $q_i$, $q_j$ and $q_m$ have the same quantity of mass, where $m$ is the index of $\max q_k, \forall k, k \neq i, k \neq j$. 

%\begin{align*}
%\frac{(1-2\eta)\beta}{2}+\eta &= (1-2\eta)(1-\beta)r\\
%\beta&=\frac{2r}{2r+1}-\frac{2\eta}{(2r+1)(1-2\eta)}
%\end{align*}
%Then, η
%we have $q_i = q_j \geq \frac{r}{2r+1}$, $q_k \leq (1-\frac{2r}{2r+1})\frac{p_k}{\Sigma_{l \neq i, j} p_l}, \forall k, k \neq i, k \neq j$. 
Hence, constructing $q$ with $\eta = \max\big(\frac{1}{2+(m_p^*/p_f)},\frac{p_i+p_j}{2}\big), q_k = p_k\frac{(1-2\eta)}{m_p^*}, \forall k \notin \lbrace i,j\rbrace$ is an optimal solution.
\end{proof}

% \newpage

\begin{lemma}
For any $0 \leq x_1 \leq x_2 \leq 1$ and $0 \leq y_2 \leq y_1 \leq 1$, \[-(x_1 \ln y_1 + x_2 \ln y_2) \geq -(\frac{x_1+x_2}{2} \ln y_1 + \frac{x_1+x_2}{2} \ln y_2) \]
\label{lemma1:v2}
\end{lemma}

\begin{proof}
\begin{align*}
-(x_1 \ln y_1 + x_2 \ln y_2) + (\frac{x_1+x_2}{2} \ln y_1 + \frac{x_1+x_2}{2} \ln y_2) &= \frac{x_2-x_1}{2} \ln y_1 - \frac{x_2-x_1}{2} \ln y_2\\
&= \frac{x_2-x_1}{2} (\ln y_1 - \ln y_2)\\
&\geq 0
\end{align*}
\end{proof}
%current
The above lemma implies that given a probability distribution $p$ with a maximum value at $j$, in order to construct a distribution $q$ whose maximum value is constrained to be at $i \neq j$ and whose cross-entropy $H(q,p)$ is minimized with respect to $q$, values in $q$ must be chosen so that the values in positions $i$ and $j$ are equal. The following theorem establishes the optimal $p$ based on these considerations.

\begin{theorem}
Given a distribution $p$, $p_j \geq p_k, \forall k$. We are asked to construct a distribution $q$ that minimizes the cross entropy $H(q,p)$ under the constraint that $q_i \geq q_k, \forall k$. Consider the  entries $l, l \neq i, l \neq j$ in $p$ that are larger than $\sqrt{p_i p_j}$. The optimal $q$ then is obtained by setting $i$, $j$, and all such entries $l$ to an equal value and all other entries in $q$ to 0.
\label{the:h_p_q}
\end{theorem}
\begin{proof}
Lemma~\ref{lemma1:v2} implies that $q_i = q_j \geq p_k, k \neq i, k \neq j$. Next, we consider which of the remaining entries in $q$ should be non-zero. Clearly, any such entry cannot exceed $q_i$. Consider when a transfer of mass $\alpha$ from $q_i$ and $q_j$ to $q_k$ reduces the entropy $H(q,p)$. For this, we must have\\
\begin{align*}
    - \alpha \ln p_k &< - (\frac{\alpha}{2} \ln p_i + \frac{\alpha}{2} \ln p_j)\\
     -  \ln p_k &< - \frac{1}{2} \ln (p_i p_j)\\
     -  \ln p_k &< - \ln \sqrt{p_i p_j}\\  
     p_k &> \sqrt{p_i p_j}\\
\end{align*}

The maximum mass that can be moved to $p_k$ cannot exceed the value $q_i$. This means that at the optimal $q$,  $q_i$, $q_j$, and all such entries $l$ for which $p_l > \sqrt{p_i p_j}$ are equal to each other, and the rest of the entries in $q$ are 0.

\end{proof}
